SliceNStitch: Continuous CP Decomposition of Sparse Tensor Streams

Consider traffic data (i.e., triplets in the form of source-destination-timestamp) that grow over time. Tensors (i.e., multi-dimensional arrays) with a time mode are widely used for modeling and analyzing such multi-aspect data streams. In such tensors, however, new entries are added only once per period, which is often an hour, a day, or even a year. This discreteness of tensors has limited their usage for real-time applications, where new data should be analyzed instantly as it arrives. How can we analyze time-evolving multi-aspect sparse data 'continuously' using tensors where time is'discrete'? We propose SLICENSTITCH for continuous CANDECOMP/PARAFAC (CP) decomposition, which has numerous time-critical applications, including anomaly detection, recommender systems, and stock market prediction. SLICENSTITCH changes the starting point of each period adaptively, based on the current time, and updates factor matrices (i.e., outputs of CP decomposition) instantly as new data arrives. We show, theoretically and experimentally, that SLICENSTITCH is (1) 'Any time': updating factor matrices immediately without having to wait until the current time period ends, (2) Fast: with constant-time updates up to 464x faster than online methods, and (3) Accurate: with fitness comparable (specifically, 72 ~ 100%) to offline methods.

==> cover_revision.tex <==
\onecolumn

\renewcommand{\thefigure}{R\arabic{figure}}
\renewcommand{\theHfigure}{R\arabic{figure}}

\begin{center}
    {\LARGE\textbf{SliceNStitch: Continuous CP Decomposition of\\ Sparse Tensor Streams}}\\
    \vspace{3mm}
    {\large Taehyung Kwon, Inkyu Park, Dongjin Lee, and Kijung Shin}
    \vspace{3mm}
\end{center}

We would like to thank the reviewers for their high quality reviews and constructive comments.
Unfortunately, we could not incorporate all suggestions within the page limit, and we had to address some in the online appendix of this paper \cite{appendix}, which is available at \blue{\url{https://bit.ly/3gJZl2u}} (a Dropbox directory without any web tracking).
Below, we summarize how we addressed the reviewers' requirements. 


 {\Large\vspace{5mm}\noindent\textbf{1.\ \ Reviewer 1}\vspace{3mm}}
\begin{itemize}[leftmargin=1em]    
	\item \textbf{R1-1. (Required Changes for a Revision)}
		\textit{``If the algorithm is designed to be effective for sparse tensors, then authors should make this clear in the title, abstract and the problem specification.
		If this is not the case and the algorithm is designed to work for both sparse and dense tensors, authors should include dense sets and other competitors designed to work for dense data in their experiments. If the algorithm is designed to work for both sparse and dense data, I recommend the authors to at least consider the data and/or algorithm in C. Ye and G. Mateos, ``Online Tensor Decomposition and Imputation for Count Data,'' 2019 IEEE Data ScienceWorkshop (DSW), Minneapolis, MN, USA, 2019''}
	
	\item \textbf{A1-1.}
		Our algorithms are indeed designed to be effective for sparse tensors, which multi-aspect data streams (Definition~\ref{defn:stream} in Section \ref{sec:problem}) are represented by.
		We clarified this fact in the title, abstract, introduction, problem definition, method, and conclusion sections of the paper.
		%Also, we would like to mention that the definition of in Section~ represents the sparseness of the data.
	
    \item \textbf{R1-2. (Required Changes for a Revision)}
          \textit{``If authors specify that their algorithm is designed to operate only for sparse data, then I would like to see a comparison against at least Gujral et al. 2018.''}
    
    \item \textbf{A1-2.}     		
   		Our response is three-fold:
   		\begin{itemize}
   			
   			\item 
   			We put a lot of effort into testing SamBaTen \cite{gujral2018sambaten} to compare our methods against it, as the reviewer suggested.
   			We first tested the official MATLAB implementation provided by the authors of the paper (\url{http://www.cs.ucr.edu/~egujr001/ucr/madlab/src/SAMBATEN.zip}).
   			Unfortunately, we could not get reasonable results, as seen in Fig.~\ref{fig:sambaten:fitness}.
   			Its fitness goes under 0 in the New York Taxi dataset and even in the sample data provided with the demo code.
   			Then, we tried hard to figure out the reason and fix potential problems, but we could not succeed within the revision period.
   			We also discussed this matter with the authors of the paper, and they will contact us as soon as they solve this issue.
   			If this issue can be solved, then we will add a comparison against SamBaTen to the final version of our paper.
   			
   			\begin{figure}[h]
   				\centering
   				\subfloat[Demo dataset]{\includegraphics[width=0.45\linewidth]{FIG/sambaten_rand_revision.pdf}\label{subfig:sambaten:demo}}
   				\subfloat[New York Taxi dataset]{\includegraphics[width=0.45\linewidth]{FIG/sambaten_nyt_revision.pdf}\label{subfig:sambaten:nyt}}
   				\caption{Fitness of SamBaTen over time.
   					\protect\subref{subfig:sambaten:demo} Result in the demo dataset `sampledata.mat', which the authors provided
   					\protect\subref{subfig:sambaten:nyt} Result in the New York Taxi dataset.
   					For fitness, we used the conventional definition in Section~\ref{sec:exp:settings}.
   				}\label{fig:sambaten:fitness}
   			\end{figure}
   			
   			\item Instead of SamBaTen, we compared our methods against two additional recent algorithms for online CP decomposition: CP-stream \cite{smith2018streaming} and NeCPD \cite{anaissi2020necpd}.
   			They are suitable as our competitors because they can handle sparse tensors, and their target is the CP decomposition based on the square loss.
   			We briefly discuss both in Section~\ref{sec:related_work:onlinecp}.
   			We reported their relative fitness over time in Fig.~\ref{fig:relative_fitness} and their average relative fitness in Fig.~\ref{fig:relative_fitness_average}.
  			We reported their update time in Fig.~\ref{fig:elapsed_time}.
  			For CP-stream, we also tested it while changing the period $T$, and the results are added to Figs.~\ref{subfig:simple_cp:fitness}, \ref{subfig:simple_cp:param}, \ref{subfig:simple_cp:time}.
  			We also tested NeCPD in the same manner and found that it  consistently provided worse trade-offs than the others.
  			In short, our proposed method \method outperformed them, providing a significantly better trade-off between speed and fitness.
  			
  			\item		 
   			We also reviewed all the papers that the reviewer mentioned and briefly discussed them in Section~\ref{sec:related}.
   			However, for comparison, we had to focus our attention to CP-stream \cite{smith2018streaming} and NeCPD \cite{anaissi2020necpd}, which we think are the most suitable competitors of our methods, due to the lack of time.    	
   			In addition, the directions of all the papers except NeCPD are slightly different from ours.
   			Specifically, Ye et al.~\cite{ye2019online} and Sobral et al.~\cite{sobral2015online} do not exploit the sparsity of the input tensor in their algorithms, while our method is designed to be effective for sparse tensors.
   			BICP~\cite{huang2016bicp} incrementally updates a block-based CP decomposition~\cite{phan2011parafac, li20162pcp}, which requires partitioned subtensors and their decompositions, rather than decompositions of the entire tensor.
   		\end{itemize}	   
   	
	\item \textbf{R1-3. (Required Changes for a Revision)}
		\textit{``I know the authors claim that this and other algorithms process every entry with the same time-mode index and therefore are not suitable for the proposed ``continuous'' problem, but I do not believe this should be a road block in devising a fair experimental comparison (e.g. by considering a time-stamp version of their algorithm and by considering a version of the existing algorithms where each data update has its won time stamp) -- In fact, looking any the data sets considered by the authors, I do not see why existing algorithms cannot be applied. I think it would be important for the authors to experimentally establish that the existing algorithms are less effective in the application domains where the data is coming from than the proposed continuous time based algorithm.''}	
		
	\item \textbf{A1-3.}	   	
		As the reviewer pointed out, by reducing the granularity of the time mode, we can reduce the update intervals of other online CPD algorithms.
		They can even handle the continuous model if the updates are made for every tensor slice defined in Definition~\ref{dfn:slice}.
		\textbf{We measured how reducing the granularity of the time mode affects the (a)  fitness, (b) parameter number, and (c) update time of CPD, OnlineSCP, and CP-stream in Fig.~\ref{fig:motivation}.}
		As seen in Figs.~\ref{subfig:simple_cp:fitness} and \ref{subfig:simple_cp:param},
		reducing the granularity significantly decreased the fitness and increased the number of parameters.
		As seen in \ref{subfig:simple_cp:time}, however, the update time did not decrease dramatically.
		As a result, \method (specifically, \hyals) in the continuous tensor model required \textbf{55$\times$ fewer parameters} while achieving \textbf{2.26$\times$ higher fitness} 
		with up to \textbf{256$\times$ shorter update times}
		than existing online algorithms for conventional CPD with extremely fine-grained time mode.
		The detailed experimental settings can be found in Section~\ref{sec:exp:continuous}.

%		In addition, it is 256 times faster than other baselines, thus more suitable for the online setting.
%		Details are included in Fig.~\ref{fig:motivation} and Section~\ref{sec:intro}.
%		Fig.~\ref{subfig:simple_cp:fitness} and \ref{subfig:simple_cp:param} clearly show the trade-off between the update interval, and fitness and the number of parameters in the baselines.	
%		Fig.~\ref{subfig:simple_cp:time} reveals that runtime per update of \method is less than that of other algorithms regardless of their update intervals.
%		Note that we don't include NeCPD because it has poor performance when using NeCPD 1 and long runtime when using NeCPD 10 (e.g. fitness-0.28 and runtime-0.24 second when the update interval is 3600).
	
	\item \textbf{R1-4.}
		(Non-required Changes) \textit{``A more extensive comparison against the state-of-the-art in online tensor decomposition.''}
		
	\item \textbf{A1-4.}
		We addressed this concern in A1-2.
		
   	\item \textbf{R1-5.}
   		(Non-required Changes)  \textit{``CP is not necessarily best decomposition model for tensor streams. The authors do not discuss alternative models, such as DEDICOM, which may be more suitable when one of the modes is time.''}
   
   	\item \textbf{A1-5.}
	As the reviewer pointed out CPD may not be the best decomposition model for tensors with time modes, and there exist a number of alternatives, including DEDICOM.
   	%Many tensor decomposition models have been widely studied, such as CP, TUCKER \cite{tucker1966some}, INDSCAL, and DEDICOM. 
   	Nevertheless, as a first step, we focus on making CPD `continuous' due to its prevalence and simplicity.
   	We leave extending our approach to more models as future work.
   	We made these facts clear in the second to last paragraph of Section~\ref{sec:intro}.
    
\end{itemize}

{\Large\vspace{5mm}\noindent\textbf{2.\ \ Reviewer 2}\vspace{3mm}}
\begin{itemize}[leftmargin=1em]
    \item \textbf{R2-1. (Required Changes for a Revision)}
	   \textit{``Include a discussion on the following theoretical works:}
	   \begin{itemize}
	   	\item Haupt, Jarvis, Xingguo Li, and David P. Woodruff. ``Near optimal sketching of low-rank tensor regression''arXiv preprint arXiv:1709.07093 (2017).
	   	\item Song, Zhao, David Woodruff, and Huan Zhang. ``Sublinear time orthogonal tensor decomposition.'' Advancesin Neural Information Processing Systems 29 (2016): 793-801.''
	   \end{itemize}
	   
	\item \textbf{A2-1.}
   		In Section~\ref{sec:related}, we included a discussion on the works suggested by the reviewer. Both works study approximation properties of some offline CP decomposition algorithms.
   		
    \item \textbf{R2-2.} (Non-required Changes)
          \textit{``If I understand correctly, SliceNStitch does not provide a theoretical guarantee on the approximation quality, which means the error can be unbounded.''}
    \item \textbf{A2-2.}
    	As the reviewer pointed out, we have not shown any theoretical guarantee on the approximation quality. To the best of our knowledge, there has been very limited work on approximation properties of online CP decomposition of tensor streams.
   	%	For the theoretical consideration, the methodologies used in offline CPD should be extended to the online version.
   		We leave analyzing approximation properties of online CP decomposition algorithms, including \method, as future work.
%   		However, we think that it is beyond the scope of our paper.
       
    \item \textbf{R2-3.} (Non-required Changes)
          \textit{``Non-experts may find it hard to understand due to the lack of running examples.''}
    \item \textbf{A2-3.}
    	  In order to help non-experts understand our work,
    	  we included an example in Fig.~\ref{fig:running_example}, which highlights the row to be updated in a factor matrix and the slice from where entries are sampled (in \hyals and \hyccd) in response to a given event.
  %  	  The selected row in the figure will be updated by \selals, \hyals, \selccd, or \hyccd.
    	  In addition, we added running examples for the final update formulas in  \selals and \hyals in Section~III of \cite{appendix}.
   % 	  Based on these illustrations, non-experts would understand up to \selals and \hyals without burdens and this will also help to figure out more difficult concepts, \selccd and \hyccd.
    \item \textbf{R2-4.} (Non-required Changes)
          \textit{``I suggest that the authors test the proposed methods on synthetic datasets with varying distributions to demonstrate each method's properties.''}
    \item \textbf{A2-4.}
    	  We performed an additional experiment on synthetic datasets with varying distributions, and the results can be found in Section~IV-A of the online appendix \cite{appendix}.
    	  In the experiment, we controlled the density of synthetic tensor streams to see how it affected the speed and fitness of different versions of \method.
    	  We showed that their empirical update time changed consistently with their theoretical time complexity.
    	  The experimental results indicate that when $p$ is small (i.e., if the density is low), it is recommended to use \selals and \selccd since they lead to shorter update times with similar fitness than \hyals and \hyccd.
    	  Conversely, when $p$ is large (i.e., if the density is high), it is recommended to use \hyals and \hyccd because their update times are shorter with similar or even higher fitness than \selals and \selccd.
\end{itemize}

{\Large\vspace{5mm}\noindent\textbf{3.\ \ Reviewer 3}\vspace{3mm}}
\begin{itemize}[leftmargin=1em]
    \item \textbf{R3-1. (Required Changes for a Revision)}
          \textit{``The motivation of the upgrading CPD for streaming data is not well justified especially against non-tensor factorization based solution such as streaming ML algorithms. I'd suggest including a discussion for this comparison and putting the motivation in a more clear way.''}
    \item \textbf{A3-1.}
		We briefly discussed the relation between tensor decomposition and machine learning in Section~\ref{sec:related_work:ml}, and we refer the reader to an extensive survey \cite{sidiropoulos2017tensor} on the topic.
		In our view, tensor decomposition and machine learning are not direct competitors. 
		Rather, they are mutually complementary.
		Specifically, CP decomposition has been a core building block of numerous machine learning (ML) algorithms, which are designed for classification \cite{rendle2010factorization}, weather forecast \cite{xu2018muscat}, recommendation \cite{yao2015context}, and stock price prediction \cite{spelta2017financial}, to name a few. Moreover, CP decomposition  has proven useful for outlier removal \cite{najafi2019outlier}, imputation \cite{shin2016fully}, and dimensionality reduction \cite{kolda2009tensor}, and thus it can be used as a preprocessing step of ML algorithms, many of which are known to be vulnerable to outliers, missings, and the curse of dimensionality. 
		By making the core building block ``real-time'', our work represents a step towards real-time ML.
		Moreover, our proposed method can directly be used as a preprocessing step of existing (non-tensor factorization-based) streaming ML algorithms.
		We clarified our view in Section~\ref{sec:related_work:ml}.
		
    \item \textbf{R3-2. (Required Changes for a Revision)}
          \textit{``The authors use the term accuracy, but actually they measure the relative performance over ALS. So accuracy on a concrete task (such as prediction) is not presented. I'd suggest including an experiment or an in-depth elaboration on the concrete effect of the performance improvement. As for this experiment any streaming data analysis task would be good. Since the authors focus on road traffic data, streaming flow classification or congestion prediction with or without the proposed method tensor decomposition.''}
    \item \textbf{A3-2.}
    	Our response is two-fold:
    	\begin{itemize}
    	  \item In Section~\ref{sec:exp:application}, we applied our algorithm and two baselines to an anomaly detection problem. 
    	  Then, we compared their precision and the average time gap between the occurrence and detection of anomalies. In short, the time gap was several orders of magnitude smaller in our algorithm than in the others, while the precision was similar in them.
    	  \item In addition, in the revision, we used the terms carefully to clearly distinguished fitness, relative fitness (i.e., relative performance over ALS), and accuracy on a concrete task (e.g., anomaly detection).
    	 \end{itemize}
   
\end{itemize}

{\Large\vspace{5mm}\noindent\textbf{4.\ \ Meta Reviewer}\vspace{3mm}}
\begin{itemize}[leftmargin=1em]
    \item \textbf{R4-1. (Required Changes for a Revision)}
          \textit{``The focus of the paper needs to be clarified: is it focusing on sparse tensors or more general? Based on this, the experimental section needs to be improved as outlined by Reviewer 1.''}
    \item \textbf{A4-1.}
    	  We addressed this concern in \textbf{A1-1}, \textbf{A1-2}, and \textbf{A1-3}.
    \item \textbf{R4-2. (Required Changes for a Revision)}
          \textit{``The paper is missing discussion of relevant papers, in particular the theoretical works as outlined by Reviewer 2.''}
    \item \textbf{A4-2.}
    	  We addressed this concern in \textbf{A2-1}.
    \item \textbf{R4-3. (Required Changes for a Revision)}
          \textit{``Better justification of extension to streaming data and an additional experiment clarifying the relative performance over ALS as outlined by Reviewer 3 is needed. As expressed in that review, the use of the term ``accuracy'' should be clarified as well.''}
    \item \textbf{A4-3.}
    	  We addressed this concern in \textbf{A3-2}.
\end{itemize}


\noindent In the submitted file, we colored \blue{blue} the parts that were added, or significantly updated. \ \\

\noindent Thank you for your consideration of this manuscript. \ \\


\noindent Sincerely, \ \\
\noindent Taehyung Kwon, Inkyu Park, Dongjin Lee, and Kijung Shin

%{\Large\vspace{5mm}\noindent\textbf{References}\vspace{3mm}}


\twocolumn
% \setcounter{section}{0}

\renewcommand{\thefigure}{\arabic{figure}}
\renewcommand{\theHfigure}{\arabic{figure}}
\setcounter{figure}{0}

